A constructive proof of dependent choice in classical arithmetic via memoization

In a recent paper, Herbelin developed dPA${^\omega}$, a calculus in which constructive proofs for the axioms of countable and dependent choices could be derived via the memoization of choice functions. However, the property of normalization (and therefore the one of soundness) was only conjectured. The difficulty for the proof of normalization is due to the simultaneous presence of dependent types (for the constructive part of the choice), of control operators (for classical logic), of coinductive objects (to encode functions of type ${\mathbb{N} \to A}$ into streams (${a_0},{a_1},...$)) and of lazy evaluation with sharing (for memoizing these coinductive objects). Elaborating on previous works, we introduce in this paper a variant of dPA${^\omega}$ presented as a sequent calculus. On the one hand, we take advantage of a variant of Krivine classical realizability that we developed to prove the normalization of classical call-by-need. On the other hand, we benefit from dL${_{\hat{tp}}}$, a classical sequent calculus with dependent types in which type safety is ensured by using delimited continuations together with a syntactic restriction. By combining the techniques developed in these papers, we manage to define a realizability interpretation \`a la Krivine of our calculus that allows us to prove normalization and soundness. This paper goes over the whole process, starting from Herbelin's calculus dPA${^\omega}$ until our introduction of its sequent calculus counterpart dLPA${^\omega}$.

==> figures/dlpaw/cps.tex <==
\centering
$\begin{array}{@{}rcl@{}}
\multicolumn{3}{l}{\text{\bf Commands}}\\
% \trl{c\tau[\reset=e]\tau'} 		& = & (\trc{c}\trenv{\tau\tau'})\,\tre{e}			\\
% \trl{c\tau}	 			& = & \trc{c}\,\trenv{\tau}				 	& \reset\notin\tau\\
\multicolumn{3}{l}{
\begin{array}{rcl}
\trc{\cmd{p}{e}}\,\tau 			& = & \trp{p}\,\tau\,\tre{e}			 	\\
\trc{\cmd{p}{\reset}}\,\tau 		& = & \trp{p}\,\tau				 	\\
\trc{\cmd{\coreset}{e}}\,\tau 		& = & \tre{e}\,\tau				 	\\
\end{array}
\qquad\qquad
\begin{array}{rcl}
\trc{\cmd{t}{\pi}}\,\tau 		& = & \trt{t}\,\tau\,\pi			 	\\
% \trc{\cmd{p}{\reset}}\tau  		& = & \lambda k.\trp{p}\,\trenv{\tau}\,k			 \\
\end{array}
}\\ [0.3em]\hline

\multicolumn{3}{l}{\text{\bf Proofs}}\\
\trp{\shift c}\,\tau\,k		& = & (\trc{c}\,\tau)\,k	 	 \\
% \trp{\shift c_t}\,\tau\,k	& = & \trct{c_t}    \,\tau[\reset,k]	 \\
\trp{\mu \alpha.c}\,\tau\,k 	& = & \trc{c}\,\tau[\alpha:=k]    \\[0.3em]

\multicolumn{3}{l}{
\begin{array}{rcl}
\trp{(p_1,p_2)}\,\tau\,k 	& = &	
\trp{p_1}\,\tau\,(\lambda \tau_1 q_1.\trp{p_2}\,\tau_1[a_1:=q_1]\,(\lambda \tau_2 q_2.k\,\tau_2[a_2:=q_2]\, \trV{(a_1,a_2)}))  \\
\end{array}
}\\
\trp{\injec{i}{p}}\,\tau\,k 					& = &	\trp{p}\,\tau\,(\lambda \tau q.k\, \tau[a:=q]\, \trV{\injec{i}{a}}) 				 \\
\trp{(t,p)}\,\tau\,k 						& = &	\trp{p}\,\tau\,(\lambda \tau.\trt{t}\,\tau\,(\lambda \tau x a.k\,\tau\, \trV{(x,a)}))	\\
% \trp{\prf p}\,\tau\,k						& = &   \trp{p}\,\tau\,(\lambda \tau q.q\,\tau\,\trf{\mut[a].\cmd{\prf a}{\reset}})	 		\\
% (\text{$\alpha$ fresh})\hfill \trp{\subst{p}{q}}\,\tau\,k 	& = &	\trp{p}\,\tau\,(\lambda \tau p'.p'\,\tau\,((\lambda \alpha.\trf{\mut[a].\cmd{\subst{a}{q}}{\alpha}})k))	\\

(\text{$a$ fresh})\hfill \trp{\cofix{t}{bx}{p}}\,\tau\,k 	& = & (\trt{t}\,\tau\,(\lambda \tau y.\trp{a}\,\tau[a:=\cpscofix{y}{bx}{\trp{p}}]))\,k 			\\
(\text{$a$ fresh})\hfill \trp{\ind{t}{p}{bx}{p_s}}\,\tau\,k 	& = & (\trt{t}\,\tau\,(\lambda \tau y.\trp{a}\,\tau[a:=\cpsind{y}{\trp{p}}{bx}{\trp{q}})])\,k 		\\[0.2em]

% \trp{()}\,\tau\,k 		& = &	k\,\tau\,\trv{()} \\
% \trp{a}\,\tau\,k 		& = &	k\,\tau\,\trv{a} \\
% \trp{\lambda x.p}\,\tau\,k 	& = &	k\,\tau\,\trv{\lambda x.p} \\
% \trp{\lambda a.p}\,\tau\,k 	& = &	k\,\tau\,\trv{\lambda a.p} \\
% \trp{\refl}\,\tau\,k 		& = &	k\,\tau\,\trv{\refl} \\
\trp{V}\,\tau\,k 		& = &	k\,\tau\,\trV{V} \\[0.3em]\hline

\multicolumn{3}{l}{\text{\bf Contexts}}\\
\multicolumn{3}{l}{
\begin{array}{rcl}
\tre{\mut a.c\tau'}\,\tau\,V	& = & \trc{c}\,(\tau[a:=V]\trenv{\tau'})\\ 
\tre{\coshift c}\,\tau\,V	& = & (\trc{c}\,\tau)\,V	 	\\
\end{array}
\qquad\qquad
\begin{array}{rcl}
\tre{\alpha}\,\tau\,V		& = & \lookup\;\alpha\,\tau\,V 		\\
\tre{f}\,\tau\,V				& = & V\,\tau\,\trf{f} \\
% && \\[0.3em]
\end{array}
}\\[0.5em]\hline 
% \tre{[]}\,\tau\,p				& = & p\,\tau\,\trf{[]} \\
% \tre{t\cdot e}\,\tau\,p				& = & p\,\tau\,\trf{t\cdot e} \\
% \tre{q\cdot e}\,\tau\,p				& = & p\,\tau\,\trf{q\cdot e} \\
% \tre{\mut (a_1,a_2).c}\,\tau\,p		& = & \trv{a}\,(\tau[a,p])\,\trf{\mut (a_1,a_2).c} \\
% \tre{\mut (x,b).c}\,\tau\,p		& = & \trv{a}\,(\tau[a,p])\,\trf{\mut (x,b).c} \\
% \tre{\mut[a_1.c_1\mid a_2.c_2]}\,\tau\,p	& = & \trv{a}\,(\tau[a,p])\,\trf{\mut [a_1.c_1\mid a_2.c_2]} \\

\multicolumn{3}{l}{\text{\bf Weak values}}\\
\multicolumn{3}{l}{
\begin{array}{rcl}
\trV{a}\,\tau\,k_v 		& = &	\lookup\;a\,\tau\,k_v \\
\end{array}
\qquad\qquad
\begin{array}{rcl}
\trV{v}\,\tau\,k_v		& = &	k_v\,\tau\,\trv{V} \\[0.3em]
\end{array}
}\\\hline

\multicolumn{3}{l}{\text{\bf Forcing contexts}}\\
\trf{t\cdot e}\,\tau\,v					& = & (\trt{t}\,\tau\,(\lambda \tau x.v\,\tau\,x))\,\tre{e} 			\\
(q_N\in\text{\nef}   )\hfill \trf{q_N\cdot e}\,\tau\,v	& = & (\trp{q_N}\,\tau\,(\lambda \tau q'.v\,\tau\,q'))\,\tre{e} 		\\
(q\notin\text{\nef})\hfill \trf{q\cdot e}\,\tau\,v	& = & \trp{q}\,\tau\,(\lambda \tau q'. v\,\tau\,q'\,\tre{e}) 			\\

(\text{$b_i$ fresh})\hfill\trf{\mut (a_1,a_2).c}\,\tau\,v			& = & \split{v}{b_1,b_2} (\trc{c}\,\tau[a_1:=b_1][a_2:=b_2]) 			\\
(\text{$b_i$ fresh})\qquad \hfill \trf{\mut [a_1.c_1\,|\,a_2.c_2]}\,\tau\,v	& = & \case{v}{b_1.\trc{c_1}\,\tau[a_1:=b_1]}{b_2.\trc{c_2}\,\tau[a_2:=b_2,]}	\\
(\text{$b$ fresh})  \hfill \trf{\mut (x,a).c}\,\tau\,v				& = & \dest{v}{y,b}(\lambda x.\trc{c})y\,\tau[a:=b]			\\
\trf{\muteq.c}\,\tau\,v				& = & \subst{v}{\trc{c}\,\tau} 								\\
\trf{[]}\,\tau\,v				& = & \exf\,v 										\\[0.3em]\hline

\multicolumn{3}{l}{\text{\bf Strong values}}\\
\multicolumn{3}{l}{
\begin{array}{rcl}

\trv{\lambda x.p}\,\tau\,V_t\,e  & = &	\trp{p}[V_t/x]\, \tau\, e 	\\
\trv{\lambda a.p}\,\tau\,V\,e & = &	\trp{p}\, \tau[a:=V]\,e 	 \\	
\trv{\refl}        	& = &	\refl 				 \\
\end{array}
    \qquad\qquad
\begin{array}{rcl}
\trv{(a_1,a_2)}    	& = &	(\trV{a_1},\trV{a_2}) 		\\
\trv{\injec{i}{a}}	& = &	\injec{i}{\trV{a}} 		 \\
\trv{(V_t,a)}        	& = &	(\trvt{V_t},\trV{a})		 \\[0.3em]
\end{array}
}         \\\hline

\multicolumn{3}{l}{\text{\bf Environments}}\\[-0.8em]
\multicolumn{3}{c}{
\hspace{-0.6em}
\begin{array}{@{}r@{~}c@{~}l}
\trenv{\tau[a:=\cofix{V_t}{bx}{p}]}	& = &	\trenv{\tau}[a:=\cpscofix{\trvt{V_t}}{bx}{\trp{p}}	 ]\\
\trenv{\tau[a:=\ind{V_t}{p}{bx}{q}]}	& = &	\trenv{\tau}[a:=\cpsind{\trvt{V_t}}{\trp{p}}{bx}{\trp{q}}]\\
\end{array}
\qquad
\begin{array}{r@{~}c@{~}l@{}}
\trenv{\varepsilon}			& = &	\varepsilon \\ 
\trenv{\tau[a:=V]}			& = &	\trenv{\tau}[a:=\trv{V}] \\
\trenv{\tau[\alpha:=e]}			& = &	\trenv{\tau}[\alpha:=\tre{e}] \\[0.8em]
\end{array}
}\\[-0.3em]\hline

\multicolumn{3}{l}{\text{\bf Terms}}\\

\trt{V_t}\,\tau\,k_t				& = & k_t\,\tau\,\trvt{V_t}\\
% \trt{0} \,\tau\,k_t 				& = & k_t\,\tau\,\trvt{0}\\
% \trt{x}\,\tau\,k_t				& = & k_t\,\tau\,\trvt{x}\\
% \trt{\lambda x.t}\,\tau\,k_t			& = & k_t\,\tau\,\trvt{\lambda x.t}\\
\trt{ S (u) }\,\tau\,k_t			& = & \trt{u}\,\tau\,(\lambda \tau x.k_t\,\tau\,\trvt{S(x)}) )					\\
\trt{t\,u}\,\tau\,k_t				& = & \trt{t}\,\tau\,\lambda \tau v.\trt{u}\,\tau\,(\lambda \tau w.v\,w\,\tau \, k_t)) 		\\
\trt{\wit(p)}\,\tau\,k_t			& = & \trp{p}\,\tau\,(\lambda \tau q.q\,\tau\,(\lambda \alpha.(\trf{\mut(x,a).\cmd{x}{\alpha}})\,k_t))	\\
% \trt{\rec{V_t} [u_0\mid (x,y).u_s])}\,\tau\,k_t & = & (\rec{V_t} [\trt{u_0}\mid (x,y).\trt{u_S}])\,\tau\,k_t					\\
\trt{\rec{t}{xy}{u_0}{u_S}}\,\tau\,k_t 	& = & \trt{t}\,\tau\,(\lambda \tau z.\rec{z}{xy}{\trt{u_0}}{\trt{u_S}}\,\tau\,k_t)	\\[0.2em]


\multicolumn{3}{l}{
\begin{array}{rcl}
% \trpi{\alpha}\,\tau\,v				& = & \alpha \, \tau\,v										 \\
\trpi{u\cdot\pi}\,\tau\,v			& = & \trt{u}\,\tau\,(\lambda \tau w. v\,\tau\,w\,\trpi{\pi})					 \\
% \trpi{\mut x. c}\,\tau\,v			& = & (\trc{c}\,\tau)[v/x]								 \\
% \trpi{\mut x. \cmd{p}{e}}\,\tau\,v		& = & (\trp{p}\,\tau\,\tre{e})[v/x]								 \\
\trpi{\mut x. c}\,\tau\,v			& = & (\trc{c}\,\tau)[v/x]								 \\
\trvt{0} 					& = & 0 		\\						      [0.2em]

\end{array}
\qquad\qquad
\begin{array}{rcl}

\trvt{x} 					& = & x 		\\
\trvt{S(V_t)}					& = & S(\trvt{V_t})	\\
\trvt{\lambda x.t} 				& = & \lambda\tau x k.\trt{t}\, \tau\, k \\
\end{array}
}\\						      
% \multicolumn{3}{l}{\text{\bf Lookup }} \\
% \multicolumn{3}{l}{
% \begin{array}{lcll}
% \lookup\,a\, (\tau_1[a,V]\tau_2)\, k_v			& \rightarrow_\beta &	V\,(\tau_1[a,V]\tau_2)\, k \\
% \lookup\,a\, (\tau_1[a,(t,x,b,p)]\tau_2)\,k_v 		& \rightarrow_\beta &	p[t/x]\,  ([b,  \lambda\tau k.k\, \tau\, (\lambda y\tau k. k (\tau[c,(y,x,b,p)]) \trv{c})]\tau_1)\,\\
% 								&	            & \qquad \qquad    (\lambda \tau q. q\, (\tau[a,q]\tau_2)\,k_v)  &\\
% % \lookup\,a\, (\tau_1[a,(t,x,b,p)]\tau_2)\,k_v 		& \rightarrow_\beta &	p[t/x]\,  ([b,  \lambda\tau k.k\, \tau\, (\lambda y\tau k. k (\tau[c,(y,x,b,p)]) \trv{c})]\tau_1)\,\\
% % 								&	            & \qquad \qquad    (\lambda \tau q. q\, (\tau[a,q]\tau_2)\,k_v)  &\\
% \lookup\,a\, (\tau_1[a,(0,p,x,b,q)]\tau_2)\,k_v 	& \rightarrow_\beta &	p \,\tau\,(\lambda \tau q. q\, (\tau_1[a,q]\tau_2)\,k_v) \\
% \lookup\,a\, (\tau_1[a,(S(t),p,x,b,q)]\tau_2)\,k_v	& \rightarrow_\beta &	q[t/x]\,(\tau_1[b,(t,p,x,b',q[b'/b])])
% 										    (\lambda \tau q. q\, (\tau_1[a,q]\tau_2)\,k_v) \\
% \end{array}
% }
\end{array}$


==> figures/dlpaw/cps_debruijn.tex <==
$$\begin{array}{rclc}
n_\tau := |\tau|+1 & & & \\

\multicolumn{4}{l}{\text{\bf Closures}}\\
\trc{\cmd{p}{e}\tau} & = & \trp{p}\,\id\,\trenv{\tau}\,\tre{e}				& \\
% \trc{\cmd{p}{e}}\,h\,tau & = & \trp{p}\,h\,\id\,\trenv{\tau}\,\tre{e}				& \\
\trc{\cmd{\shift c_\reset}{e}\tau} & = & (\trc{c_\reset}\,\trenv{\tau})\,\tre{e}	& \\
\trc{\cmd{p}{\reset}}\,h\, \tau & = & \lambda k.\trp{p}\,h\,\tau\,k				& \\

\multicolumn{4}{l}{\text{\bf Proofs}}\\


\trp{\mu \alpha.c}\, h\,\tau\,k 	& = &	\trc{c[k/\alpha]} \,\tau& \\[0.5em]

\trp{(p_1,p_2)}\, h\,\tau\,k 		& = &	\trp{p_1}\, h\,\tau\,(\lambda h_1\tau_1 q_1.\trp{p_2}\, (h_1\circ h)\,(\tau_1[\flagv,q_1])\,
							    (\lambda h_2\tau_2 q_2.k\,(h_2\circ h_1)\,(\tau_2[\flagv,q_2])\, \flagv\, \trv{(n_{\tau_1},n_{\tau_2})})) & \\
\trp{\injec{i}{p}}\, h\,\tau\,k 	& = &	\trp{p}\,h \,\tau\,(\lambda h_p\tau_p q.k\,h_p \tau_p[\flagv,q]\, \trv{\injec{i}{n_{\tau_p}}}) 				& \\
\trp{(t,p)}\, h\,\tau\,k 		& = &	\trp{p}\,h\,\tau_p\,(\lambda h_p\tau_p q.\trt{t}\,(h_p\circ h)\,\tau_p[\flagv,q]\,
(\lambda h_t \tau_t u. k\,(h_p\circ h_t)\,\tau_t\, \trv{(u,n_{\tau_p})}))	& \\
\trp{\prf p}\, h\,\tau\,k		& = &   (\trp{p}\, h \,\tau\,(\lambda h_p \tau_p q.q\,\id\,(\tau_p[\flagv,q])(\lambda h_q\tau_q v.\trf{\prf{\bullet}} h_q\,\tau_q\, v)))k&\\
% \lookup\,a~(\tau[a,\flagv,p'])\,\trf{\prf \,{\bullet}})) )\,k	& \\
\trp{\subst{p}{q}}\, h\,\tau\,k 	& = &	\trp{p}\,\tau\,(\lambda h_p \tau_p p'.p'\id \,h_p\,\tau_p\,(\lambda h. k (h\circ h_p)) )		& \\[0.2em]

\trp{\cofix{t}{x,b}{p}}\, h\,\tau\,k 	& = & \trt{t}\,\tau\,(\lambda \tau y. k\,(\tau[\flagc,(y,x,b,\trp{p})])\,\trv{n_\tau}) 		& \\
\trp{\ind{t}{p_0}{x,a}{p_s}}\, h\,\tau\,k 	& = & \trt{t}\,\tau\,(\lambda \tau x.k\,(\tau[\flagi,(y,\trp{p_0},x,b,\trp{p_S})])\,\trv{n\tau} )	&  \\[0.2em]

% \trp{()}\, h\,\tau\,k 			& = &	k\,\id\,\tau\,\trv{()} \\
% \trp{a}\, h\,\tau\,k 			& = &	k\,\id\,\tau\,\trv{a} \\
% \trp{\lambda x.p}\, h\,\tau\,k	 	& = &	k\,\id\,\tau\,\trv{\lambda x.p} \\
% \trp{\lambda a.p}\, h\,\tau\,k 		& = &	k\,\id\,\tau\,\trv{\lambda a.p} \\
% \trp{\refl}\, h\,\tau\,k 		& = &	k\,\id\,\tau\,\trv{\refl} \\
\trp{V}\, h\,\tau\,k 			& = &	k\,\id\,\tau\,\trv{V} & \\[0.3em]

\multicolumn{4}{l}{\text{\bf Contexts}}\\
\tre{\alpha}\,h\,\tau\,p			& = & \alpha\,\id\,\tau\,p & \\
\tre{\mut a.c\tau'}\,h\,\tau\,p			& = & \trc{c[n_\tau/a]}\,\id\,(\tau[\flagv,p]\trenv{\tau'}) & \\
\tre{f}\,h\,\tau\,p				& = & p\,\id\,\tau\,\trf{f}^h & \\

% \tre{[]}\,h\,\tau\,p				& = & p\,\id\,\tau\,\trf{[]} & \\
% \tre{\alpha}\,h\,\tau\,p			& = & \alpha\,\id\,\tau\,p & \\
% \tre{\mut a.c\tau'}\,h\,\tau\,p		& = & \trc{c}\,\id\,\tau[a,\flagv,p]\trenv{\tau'} & \\
% \tre{t\cdot e}\,h\,\tau\,p			& = & p\,\id\,\tau\,\trf{t\cdot e} & \\
% \tre{q\cdot e}\,h\,\tau\,p			& = & p\,\tau\,\trf{q\cdot e} & \\
% \tre{\mut (a_1,a_2).c}\,h\,\tau\,p		& = & p\,\id\,\tau\,\trf{\mut (a_1,a_2).c} & \\
% \tre{\mut (x,b).c}\,h\,\tau\,p		& = & p\,\id\,\tau\,\trf{\mut (x,b).c} & \\
% \tre{\mut[a_1.c_1\mid a_2.c_2]}\,h\,\tau\,p	& = & p\,\id\,\tau\,\trf{\mut [a_1.c_1\mid a_2.c_2]} & \\

\multicolumn{4}{l}{\text{\bf Values}}\\
\trv{()}\, h\,\tau\,k_v 		& = &	k_v\,\tau\,\flagv\,\trv{()} & \\
\trv{n}\, h\,\tau\,k_v 		& = &	\lookup\,h(n)\,\tau\,k_v & \\
\trv{\lambda x.p}\, h\,\tau\,k_v 	& = &	k_v\,\tau\,\lambda x .\trp{p} & \\ 
\trv{\lambda a.p}\, h\,\tau\,k_v 	& = &	k_v\,\tau\,(\lambda q \tau k.\trp{p}\,\tau[a,\flagv,q]\,k) & \\
\trv{(a_1,a_2)}\, h\,\tau\,k_v 	& = &	k_v\,\tau\,(\trv{a_1},\trv{a_2})) & \\
\trv{\injec{i}{a}}\, h\,\tau\,k_v 	& = &	k_v\,\tau\,\injec{i}{\trv{a}} & \\
\trv{(t,a)}\, h\,\tau\,k_v 		& = &	k_v\,\tau\,(t,\trv{a}) & \\
\trv{\refl}\, h\,\tau\,k_v 		& = &	k_v\,\tau\,\refl & \\



\multicolumn{4}{l}{\text{\bf Forcing Contexts}}\\
\trf{[]}^h\,h'\,\tau\,v					& = & \exf\,v(\,\tau ??) & \\
\trf{\mut[a].\cmd{a}{f}\tau'}^h\,h'\,\tau\,v		& = & \trf{f}^h\,h'\,(\tau[\flagv,v](\mapop (h'\circ  h)\, \trenv{\tau'})\,v & \\
\trf{\mut[a].\cmd{\prf a}{\reset}}^h\,h'\,\tau\,v	& = & \lambda k. k\,(h'\circ h)\,(\tau[\flagv,v])\,(\snd v)\\
\trf{\mut[a].\cmd{\subst{a}{q}}{e}}^h\,h'\,\tau\,v 	& = & \subst{v}{\trp{q}}\,(h'\circ h)\,\tau[\flagv,v]\,(\lambda h''.k (h''\circ h'\circ h))\\
\trf{t\cdot e}^h\,h'\,\tau\,v				& = & \trt{t}\,(h'\circ h)\,\tau\,(\lambda h_t \tau u. v\,u\,(h_t\circ h'\circ h)\,\tau\,\tre{e}) & \\
\trf{q\cdot e}^h\,h'\,\tau\,v				& = & \trp{q}\,(h'\circ h)\,\tau\,(\lambda h_q \tau q. v\,q\,(h_q\circ h'\circ h)\,\tau\,\tre{e}) & \\
\trf{q\cdot e}^h\,h'\,\tau\,v				& = & \trp{q}\,(h'\circ h)\,\tau\,(\lambda h_q \tau q. v\,q\,(h_q\circ h'\circ h)\,\tau\,\tre{e}) & \\
\trf{\mut (a_1,a_2).c\tau'}^h\,h'\,\tau\,v		& = & \split{v}{a_1,a_2} \trc{c[n_\tau/a_2][n_\tau+1/a_1]}\,(h'\circ h)\, (\tau[\flagv,a_2][\flagv,a_1])& \\
\trf{\mut (x,b).c\tau'}^h\,h'\,\tau\,v			& = & \dest{v}{x,b}\trc{c[n_\tau/b]}\,(h'\circ h)\,\tau[\flagv,b]& \\
\trf{\mut [a_1.c_1\mid a_2.c_2]}^h\,h'\,\tau\,v		& = & \case{v}{a_1.\trc{c_1[n_\tau/a_1]}\,(h'\circ h)\,\tau[\flagv,a_1]}{a_2.\trc{c_2[n_\tau/a_2]}\,(h'\circ h)\,\tau[\flagv,a_2]} & \\


\multicolumn{4}{l}{\text{\bf Environments}}\\
\trenv{\tau[a=V]}				& = &	\trenv{\tau}[\flagv,\trv{V}] & \\
\trenv{\tau[a=\cofix{V_t}{x,b}{p}]}		& = &	\trenv{\tau}[\flagc,(\trvt{V_t},x,b,\trp{p})]& \\
\trenv{\tau[a=\ind{V_t}{p_0}{x,b}{p_S}]}	& = &	\trenv{\tau}[\flagi,(V_t,\trp{p_0},x,b,\trp{p_S})]& \\
\trenv{\varepsilon}				& = &	\varepsilon & \\ 

\multicolumn{4}{l}{\text{\bf Terms}}\\

\trt{0} \,h\,\tau\,k_t 				& = & k_t\,h\,\tau\,0& \\
\trt{ S (u) }\,h\,\tau\,k_t			& = & \trt{u}\,h\,\tau\,(\lambda h\tau x.k_t\,h\,\tau\,S(x)) )& \\
\trt{x}\,h\,\tau\,k_t				& = & k_t\,h\,\tau\,x& \\
\trt{\lambda x.t}\,h\,\tau\,k_t			& = & k_t\,h\,\tau\,\lambda x.(\lambda h\tau k_t.\trt{t} h \tau k_t)& \\
\trt{t\,u}\,h\,\tau\,k_t				& = & \trt{u}\,h\,\tau\,(\lambda h\tau x.\trt{t}\,h\,\tau\,(\lambda h\tau y.y\,x\,h\,\tau \, k_t))& \\
\trt{\wit(p)}\,h\,\tau\,k_t			& = & \trp{p}\,h\,\tau\,(\lambda h \tau f q .q\,h\,\tau[a,f,q]\,(\lambda h \tau b.\pi_1(b)\,h\,\tau)) & \\
\trt{\rec{t} [u_0\mid (x,y).u_s])}\,h\,\tau\,k_t   & = & \trt{t}\,h\,\tau\,(\lambda h \tau x.
						      \trt{u_0}\,h\,\tau\,(\lambda h \tau y_0.
						      \trt{u_S}\,h\,\tau\,(\lambda h \tau y_S.k_t\,h\,\tau\,\rec{x} [y_0\mid (x,y).u_s])))& \\
						      
% \multicolumn{4}{l}{\text{\bf Lookup  (manque $\alpha$-conversion \'a la vol\'ee}} \\
% \multicolumn{4}{l}{
% \begin{array}{lcll}
% \lookup\,a\,(\tau_1[a,\flagv,V]\tau_2)\, k_v			& \rightarrow_\beta &	V\,(\tau_1[a,\flagv,V]\tau_2)\, k \\
% \lookup\,a\,(\tau_1[a,\flagc,(t,x,b,p)]\tau_2)\,k_v 		& \rightarrow_\beta &	p[t/x]\,  ([b,\flagv,  \lambda\tau k.k\, \tau\, (\lambda y\tau k. k (\tau[c,\flagc,(y,x,b,p)]) \trv{c})]\tau_1)\,\\
% 								&	            & \qquad \qquad    (\lambda \tau q. q\, (\tau[a,\flagv,q]\tau_2)\,k_v)  &\\
% \lookup\,a\,(\tau_1[a,\flagi,(0,p_0,x,b,p_S)]\tau_2)\,k_v 	& \rightarrow_\beta &	p_0 \,\tau\,(\lambda \tau q. q\, (\tau_1[a,\flagv,q]\tau_2)\,k_v) \\
% \lookup\,a\,(\tau_1[a,\flagi,(S(t),p_0,x,b,p_S)]\tau_2)\,k_v	& \rightarrow_\beta &	p_S[t/x]\,(\tau_1[b,\flagi,(t,p_0,x,b',p_S[b'/b])])
% 										    (\lambda \tau q. q\, (\tau_1[a,\flagv,q]\tau_2)\,k_v) \\
% \end{array}
% }
\end{array}$$



==> figures/dlpaw/old-types.tex <==

{\bf Regular types} \vspace{-0.7em}
$$
\begin{array}{c}
%  \infer[\tau_I]{\sigmaopt\Gamma\vdash c[a=p]\tau}{\sigmaopt\Gamma,a=p \vdash c\tau} 
%  \qquad
%  \infer[\tau_E]{\sigmaopt\Gamma,a = p_\tau ,\Delta \vdash p:A}{\sigmaopt\Gamma \vdash p[p_\tau/a]:A} 
%  \qquad
% %  \infer[conv^-]{\sigmaopt\Gamma \vdash e: B^\negt;\eps}{\sigmaopt\Gamma\vdash e: A^\negt & A\equiv B}
%  \infer[\textsc{Cut}]{\sigmaopt\Gamma\vdash \cmd{p}{e}}{
%       \sigmaopt\Gamma,\tau \vdash p:A & \sigmaopt\Gamma,\tau \vdash e:A^\negt 
%      } 
% \\
% \\
\infer[\tauprule]{\sigmaopt\Gamma\sigdash \tau[a:=p]:(\Gamma',a:A;\sigma'\dpt{a|p})}{\sigmaopt\Gamma \sigdash \tau:(\Gamma';\sigma') & \sigsigprimeopt\Gamma,\Gamma' \sigsigdash p :A }
 \qquad\quad
\infer[\tauerule]{\sigmaopt\Gamma\sigdash \tau[\alpha:=e]:(\Gamma',\alpha:A^\negt;\sigma') }{\sigmaopt\Gamma \sigdash \tau:(\Gamma';\sigma') & \sigsigprimeopt\Gamma,\Gamma' \sigsigdash \alpha :A^\negt }
% \qquad
% \infer[\tautprule]{\sigmaopt\Gamma\vdash_d c\tau[\reset:=e]:\sigmaopt\Gamma',\reset:A^\negt;\eps}{\sigmaopt\Gamma \vdash \tau:\sigmaopt\Gamma' & \sigmaopt\Gamma,\sigmaopt\Gamma' \vdash e :A^\negt  } 
 
\\[0.8em]


%  \infer[\tauprule]{\sigmaopt\Gamma\vdash c\tau[a:=p]}{\sigmaopt\Gamma,a:A \vdash c\tau & \sigmaopt\Gamma \vdash p :A }
%  \qquad
%  \infer[\tauerule]{\sigmaopt\Gamma\vdash c\tau[\alpha:=e]}{\sigmaopt\Gamma,\alpha:A^\negt \vdash c & \sigmaopt\Gamma \vdash e :A^\negt } 
%  \qquad
%  \infer[\tautprule]{\sigmaopt\Gamma\vdash c\tau[\reset:=e]}{\sigmaopt\Gamma,\reset:A^\negt \vdash_d c\tau;\eps & \sigmaopt\Gamma \vdash e :A^\negt  } 
%  
%  
%  \\\\
 

\infer[\cutrule]{\sigmaopt\Gamma\sigdash \cmd{p}{e}\optsigma}{
      \sigmaopt\Gamma \sigdash p:A \optsigma& \sigmaopt\Gamma \sigdash e:B^\negt \optsigma
      & \sigma(A) = \sigma(B)
     } 
\qquad\quad
\infer[\lrule]{\sigmaopt\Gamma\vdash c\tau}{
      \sigsigprimeopt\Gamma,\Gamma' \sigsigdash c & \sigmaopt\Gamma \sigdash \tau:(\Gamma';\sigma')
     }

 
\\[0.5em]

 
\infer[\axrrule]{\sigmaopt\Gamma\sigdash a:A\optsigma}{(a : A)\in\Gamma}
\qquad\quad
\infer[\axlrule]{\sigmaopt\Gamma \sigdash \alpha :A^\negt\optsigma}{(\alpha : A^\negt)\in\Gamma} 
 \qquad\quad
\infer[\murule]{\sigmaopt\Gamma \sigdash \mu\alpha.c : A \optsigma}{\sigmaopt\Gamma,\alpha:A^\negt\sigdash c\optsigma}
% \qquad\quad
\\[0.8em]
\infer[\mutrule]{\sigmaopt\Gamma \sigdash \mut a.c\tau : A^\negt\optsigma}{\sigmaopt\Gamma,a:A\sigdash c\tau\optsigma}
\qquad\quad
\infer[\andrrule]{\sigmaopt\Gamma \sigdash (p_1,p_2) : A\wedge B\optsigma}{\sigmaopt\Gamma \sigdash p_1: A\optsigma  & \sigmaopt\Gamma \sigdash p_2:B\optsigma}
\qquad\quad
\infer[\andlrule]{\sigmaopt\Gamma \sigdash \mut(a_1,a_2). c: (A_1\wedge A_2)^\negt\optsigma}{\sigmaopt\Gamma, a_1:A_1, a_2:A_2\sigdash c\optsigma}
\\[0.8em]
\infer[\orrrule]{\sigmaopt\Gamma \sigdash \injec{i}{p} : A_1\vee A_2\optsigma }{\sigmaopt\Gamma \sigdash p: A_i \optsigma}
\qquad\qquad
\infer[\orlrule]{\sigmaopt\Gamma \sigdash \mut[a_1.c_1\mid a_2.c_2]:(A_1\lor A_2)^\negt\optsigma}{\sigmaopt\Gamma, a_1:A_1\sigdash c_1& \sigmaopt\Gamma, a_2:A_2\sigdash c_2\optsigma}
\\[0.8em]
  
\infer[\exrrule]{\sigmaopt\Gamma \sigdash (t,p) : \exists x^T.A \optsigma}{\sigmaopt\Gamma \sigdash p: A[t/x] \optsigma & \sigmaopt\Gamma \sigdash t:T \optsigma}
\qquad\qquad
 \infer[\exlrule]{\sigmaopt\Gamma \sigdash \mut (x,a).c: (\exists x^T. A)^\negt\optsigma }{\sigmaopt\Gamma, x:T, a:A\sigdash c\optsigma}
 \\[0.8em]  
 
 \infer[\farrule]{\sigmaopt\Gamma \sigdash \lambda x.p : \forall x^T. A\optsigma }{\sigmaopt\Gamma,x:T \sigdash p: A\optsigma }
 \qquad
 \infer[\falrule]{\sigmaopt\Gamma \sigdash t\cdot e : (\forall x^T. A)^\negt\optsigma }{\sigmaopt\Gamma \sigdash t : T\optsigma  & \sigmaopt\Gamma \sigdash e : A[t/x]^\negt\optsigma }
 \qquad
 \infer[\refl]{\sigmaopt\Gamma \sigdash \refl : t=t\optsigma }{\sigmaopt\Gamma \sigdash t : \N\optsigma }
 \\[0.8em]
 
 
   \infer[\eqrule]{\sigmaopt\Gamma \sigdash \muteq.\cut{p}{e} : (t=u)^\negt\optsigma }{\sigmaopt\Gamma \sigdash p:A\optsigma & \sigmaopt\Gamma \sigdash e : A[u/t]\optsigma}	
    \qquad
  \infer[\convrrule]{\sigmaopt\Gamma \sigdash p: B\optsigma }{\sigmaopt\Gamma\sigdash p: A\optsigma & A \equiv B}
\qquad
\infer[\convlrule]{\sigmaopt\Gamma \sigdash e: B^\negt \optsigma}{\sigmaopt\Gamma\sigdash e: A^\negt & A \equiv B}
\\[0.8em]

\infer[\imprrule]{\sigmaopt\Gamma \sigdash \lambda a.p : \dptprod{a:A} B\optsigma}{\sigmaopt\Gamma,a:A \sigdash p : B\optsigma}
 \qquad\quad
 \infer[\implrule]{\sigmaopt\Gamma \sigdash q\cdot e : (\dptprod{a:A} B)^\negt\optsigma}{
	    \sigmaopt\Gamma \sigdash q : A \optsigma
	    & 
	    \sigmaopt\Gamma \sigdash e : B[q/a]^\negt\optsigma
	    & \text{if } q\notin \text{\nef} \text{ then } a\notin A
	   }
  \\[0.8em]


 \infer[\bot]{\sigmaopt\Gamma\sigdash []:\bot^\negt\optsigma}{}  
 \qquad\qquad
   \infer[\indrule]{\sigmaopt\Gamma\sigdash \ind{t}{p_0}{ax}{p_S} : A[t/x]\optsigma}{
	  \sigmaopt\Gamma\sigdash t: \N  \optsigma
	  &
	  \sigmaopt\Gamma \sigdash p_0:A [0/x]  \optsigma
	  &
	  \sigmaopt\Gamma,x:T,a:A\sigdash p_S:A[S(x)/x]\optsigma
	}


  \\[0.8em]
  \infer[\cofixrule]{\sigmaopt\Gamma\sigdash \cofix{t}{bx}{p}: \nu^t_{fx} A \optsigma}{
	\sigmaopt\Gamma\sigdash t:T  \optsigma
	& 
	\sigmaopt\Gamma, f:T\imp \N,x:T,b:\forall y^T\!. f(y)=0\sigdash p:A  \optsigma
	& 
	f\text{ positive in } A
  }
 \end{array}   \vspace{-0.8em}
$$  
% \vspace{-1.2em}

\hrulefill\\
{\bf Dependent mode}\vspace{-0.7em}
%   \newcommand{\dpt}[1]{\{#1\}}
%   \newcommand{\eps}{\varepsilon}
% \hfill
% $A[p/\bullet]_{\eps\dpt{p|q}} := A[q/\bullet]_{\eps}, q\notin \text{Nef} \imp \bullet\notin A $~
$$
\begin{array}{c@{\quad}c}
 \infer[ \shiftrule]{\Gamma\sigdash \shift c_\reset : A}{
\Gamma,\reset:A^\negt\vdash_d c_\reset;\sigma
  }
&
\infer[\resetrule]{\Gamma,\reset : A^\negt,\Gamma' \vdash_d \reset:B^\negt;{\sigma\dpt{\cdot|p}}}{\sigma(A)=\sigma(B)}
\\[0.8em]

\infer[\dlrule]{\Gamma \vdash_d c_\reset\tau;\sigma}{\Gamma,\Gamma'\vdash_d c_\reset;\sigma\sigma' & \Gamma\sigdash \tau:(\Gamma';\sigma')}
&
\quad\infer[\dcutrule]{\Gamma,\reset:B^\negt,\Gamma' \vdash_d \cmd{p}{e};\sigma}{\Gamma,\Gamma'\sigdash {p}:{A}  & \Gamma,\reset:B^\negt,\Gamma'\vdash_d e:A^\negt;\sigma\dpt{\cdot|p} }

\\[0.8em]


% \infer[\dtauprule]{\Gamma\vdash_d \tau[a:=p]:(\Gamma',a:A;\sigma\dpt{a|p})}{\Gamma \vdash_d \tau:(\Gamma';\sigma) & \Gamma,\Gamma' \vdash p:A}
% &
% \infer[\dtauerule]{\Gamma\vdash_d \tau[\alpha:=e]:(\Gamma',\alpha:A^\negt;\sigma)}{\Gamma \vdash_d \tau:(\Gamma';\sigma) & \Gamma,\Gamma' \vdash e:A^\negt}
% % 
% % \infer[\tau_\reset]{\Gamma\vdash_d c[\reset=e]\tau}{\Gamma,\reset:A^\negt \vdash_d c\tau & \Gamma \vdash e :A^\negt  } 
% % \qquad	
% \\[0.8em]

 
\infer[\dmutrule]{\Gamma \vdash_d {\mut a.c_\reset\tau'} : A^\negt ;{\sigma\dpt{\cdot|p_N}}}{\Gamma,{a}:{A} \vdash_d c_\reset\tau';{\sigma\dpt{a|p_N}}}
 &
\infer[\dexlrule]{\Gamma \vdash_d \mut (x,a).c_\reset: (\exists x^T A)^\negt  ;\sigma\dpt{\cdot|p_N}}{\Gamma, x:T, a:A\vdash_d c_\reset;\sigma\dpt{(x,a)|p_N}}
 \\[0.8em]
  
  \infer[\dandlrule]{\Gamma \vdash_d \mut(a_1,a_2). c_\reset: (A_1\wedge A_2)^\negt;\sigma\dpt{\cdot|p_N}}{
       \Gamma, a_1:A_1, a_2:A_2\vdash_d c_\reset;\sigma\dpt{(a_1,a_2)|p_N}
       }
  &
  \infer[\dorlrule]{\Gamma \vdash_d \mut[a_1.c_\reset^1\mid a_2.c_\reset^2]:(A_1\lor A_2)^\negt;\sigma\dpt{\cdot|p_N}}{
       \Gamma, a_i:A_i\vdash_d c_\reset^i ;\sigma\dpt{\injec{i}{a_i}|p_N})
       & \forall i\in\{1,2\} }\\

 
 \end{array}\vspace{-0.1em}$$



\hrulefill\\	
   {\bf Terms}\vspace{-0.5cm}
$$\begin{array}{c}
 \infer[\autorule{0}]{\sigmaopt\Gamma\sigdash 0:\N  }{}
 \qquad
 \infer[\!\autorule{S}]{\sigmaopt\Gamma\sigdash S(t): \N }{\sigmaopt\Gamma \sigdash t:\N } 
 \qquad
 \infer[\!\lamrule]{\sigmaopt\Gamma \sigdash \lambda x.t : U\imp T}{\sigmaopt\Gamma,x:U\sigdash t:T} 
 \qquad
 \infer[\!\apprule]{\sigmaopt\Gamma \sigdash t~u : T}{\sigmaopt\Gamma\sigdash t: U\imp T & \sigmaopt\Gamma\sigdash u:U}
 \\[0.8em]
 
 \infer[\!\axxrule]{\sigmaopt\Gamma\sigdash x:T}{(x:T)\in\sigmaopt\Gamma} 
  \quad
 \infer[\!\autorule{\texttt{rec}}]{\sigmaopt\Gamma\sigdash \rec{t}{xy}{t_0}{t_S} : U}{
	\sigmaopt\Gamma\sigdash t:\N  
	& 
	\sigmaopt\Gamma\sigdash t_0:U  
	&
	\sigmaopt\Gamma,x:\N,y:U\sigdash t_S:U 
  }
  \quad
  \infer[\!\witrule]{\sigmaopt\Gamma \sigdash \wit p : T}{
	\sigmaopt\Gamma \sigdash p: \exists x^T\!.A  
	&
	p \textrm{  \nef}
  }
 \end{array}\vspace{-0.8em}
$$ 


==> figures/dlpaw/smallstep.tex <==
\setlength{\saut}{0.5em}
\newcommand{\mytitle}[1]{\multicolumn{3}{l}{\textrm{\bf #1 }} \\[0.3em]}

\centering 
$\begin{array}{r@{~}c@{~}l}
  \mytitle{Commands}
    \cut{p}{e}_c\tau 	& \reds & \cut{p}{e}_p \\
    \cut{t}{\pi}_c\tau 	& \reds & \cut{t}{\pi}_t \\[0.5em]\hline
    
    
%%%%%%%%%%%% DELIMITED CONTINUATIONS %%%%%%%%%%%%%%%%%%%%%%%%%%    
   \multicolumn{3}{l}{\textrm{\bf Delimited continuations}} \\[0.3em]
\text{(for any $\iota,o$)} \hfill		\cmd{\shift c\tau''}{e}_p\tau   &\reds& \cmd{\shift c'\tau''}{e}_p\tau'\hfill(\text{if } c_\iota\tau \reds c'_o\tau')     	\\	
% 		  \cut{\shift\cmd{p}{\alpha}}{e}_p\tau[\alpha:=\reset]\tau'	& \reds       & \cmd{p}{e}_p\tau[\alpha:=e]\tau'						\\
			\cut{\shift\cmd{p}{\reset}}{e}_p\tau			& \reds       & \cmd{p}{e}_p\tau								\\
% 			    \cut{\shift\cmd{p}{\reset}\tau'}{e}_p\tau		& \reds       & \cmd{p}{e}_p\tau\tau'								\\
\text{(for any $\iota,o$)}\hfill  \cmd{V}{\coshift c}_e\tau &\reds& \cmd{V}{\coshift c'}_e\tau' \hfill (\text{if } c_\iota\tau \reds c'_o\tau')     		\\	
				\cut{V}{\coshift\cmd{\coreset}{e}}_e\tau	& \reds       & \cmd{V}{e}_e\tau							\\[0.5em]\hline
%  \\[-1em]

%   \multicolumn{3}{l}{\textrm{\bf Delimited continuations}}\\
%   \reset\notin \tau' \hfill \cmd{p}{\reset}_\reset\tau[\reset = e]\tau' 	& \cmd{p}{e}_p\tau\tau'          \\
%   \cmd{p}{e}_\reset\tau& \reds & \cmd{p}{e}_p\tau\tau' 					 \\[0.5em]\hline


%%%%%%%%%%%%%% PROOFS %%%%%%%%%%%%%%%%%%%%%
  \mytitle{Proofs}\\[-2.4em]&&\hfill(\text{where $a,y$ are fresh}) \\
  (e\neq e_\reset)\hfill \cmdp{\mu \alpha.c}{e}\tau  			& \reds & c_c\,\tau[\alpha:=e]			 		\\
  \cmdp{\mu \alpha.c}{e_\reset}\tau  					& \reds & c_c[e_\reset/\alpha]\,\tau			 				\\[0.3em]

  \cmdp{(p_1,p_2)}{e}\tau    			& \reds & \cmdp{p_1}{\mut a_1.\cmd{p_2}{\mut a_2.\cmd{(a_1,a_2)}{e}}}\tau	 	 \\
  \cmdp{\injec{i}{p}}{e}\tau 			& \reds & \cmdp{p}{\mut a.\cmd{\injec{i}{a}}{e}}\tau 					 \\
  \cmdp{(t,p)}{e}\tau        			& \reds & \cmdp{p}{\coshift \cmd{t}{\mut x.\cmd{\coreset}{\tmu a.\cut{(x,a)}{e}}}}\tau 	 \\[0.3em]

  \cmdp{\ind{t}{p}{bx}{q}}{e}\tau	 	& \reds & \cmdp{\shift\cmd{t}{\mut y.\cmd{a}{\reset}[a:=\ind{y}{p}{bx}{q}]}}{e}\tau \\
  \cmdp{\cofix{t}{bx}{p}}{e}\tau          	& \reds & \cmdp{\shift\cmd{t}{\mut y.\cmd{a}{\reset}}[a:=\cofix{y}{bx}{p}]}{e}\tau \\[0.3em]


  \cmdp{V}{e}\tau            			& \reds & \cmde{V}{e} 								 \\[0.5em]\hline

  
%%%%%%%%%%%%%% CONTEXTS %%%%%%%%%%%%%%%%%%%%%  
  \multicolumn{3}{l}{\text{\bf Contexts}}\\
  \cut{V}{\alpha}_e\tau[\alpha := e]\tau' 	& \reds& \cut{V}{e}_e\tau[\alpha := e]\tau'	\\
  \cmde{V}{\mut a.c\tau'}\tau			& \reds & c_c\tau[a:=V]\tau' 				 \\
%   \cmde{V}{\mut a.c_t\tau'}\tau			& \reds & c_t\tau[a:=V]\tau' 				 \\
  \cmde{V}{f}\tau 				& \reds & \cmd{V}{f}_V\tau 				 \\[0.5em]\hline  

%%%%%%%%%%%%%% VALUES %%%%%%%%%%%%%%%%%%%%%
  \multicolumn{3}{l}{\text{\bf Values}}\\[-1em]&&\hfill(\text{where $b'$ is fresh}) \\
 
  \cmd{a}{f}_V\tau[a:=V]\tau'				& \reds & \cmd{V}{f}_V\tau[a:=V]\tau' 								 \\
%   \cmdv{a}{f}\tau'[a=p]\tau 				& \reds & \cmdp{p}{\mut [a].\cmd{a}{f}\tau'}\tau 						& \reds & (p\textrm{ not a value (ie cofix/ind)})\\
   \cmd{v}{f}_V\tau					& \reds & \cmdf{v}{f}\tau 									\\[0.3em]
   		          \cmd{a}{f}_V\tau[a=\ind{0}{p_0}{bx}{p_S}]\tau'		& \reds & \cmdp{p_0}{\mut a.\cmd{a}{f}\tau'}\tau         						 \\
   \cmdv{a}{f}\tau[a=\ind{S(t)}{p_0}{bx}{p_S}]\tau' 	& \reds & \cmdp{p_S[t/x][b'/b]}{\mut a.\cmd{a}{f}\tau'}\tau[b':=\ind{t}{p_0}{bx}{p_S}]]\\[0.5em]
   \cmd{a}{f}_V\tau[a=\cofix{t}{bx}{p}]\tau'		& \reds & \cmdp{p[t/x][b'/b]}{\mut a.\cmd{a}{f}\tau'}\tau[b':=\lambda y.\cofix{y}{bx}{p}] 	\\[0.3em]\hline

  
%%%%%%%%%%%%%% FORCING CONTEXTS %%%%%%%%%%%%%  
  \multicolumn{3}{l}{\text{\bf Forcing contexts}} \\[-0.5em]
  
%   \cmdf{(V_t,V)}{\mut[a].\cmd{\wit a}{\pi}}\tau 			& \reds & \cmdpi{V_t}{\pi}\tau	 			 \\
%   \cmdf{(V_t,V)}{\mut[a].\cmd{\prf{a}}{\reset}}\tau			& \reds & \cmdp{V}{\reset}\tau 				 \\
  

    
%   \cmdf{\lambda x.p}{t\cdot e}\tau 					& \reds & \cmdp{p[t/x]}{e}\tau 			& \reds & \\
  \cmdf{\lambda x.p}{t\cdot e}\tau 					& \reds & \cmdp{\shift\cmd{t}{\mut x.\cmd{p}{\reset}}}{e}\tau 	 \\
    (q\in\text{\nef}   )\hfill \cmdf{\lambda a.p}{q\cdot e}\tau 	& \reds & \cmdp{\shift\cmd{q}{\mut a.\cmd{p}{\reset}}}{e}\tau 	 \\
    (q\notin\text{\nef})\hfill \cmdf{\lambda a.p}{q\cdot e}\tau 	& \reds & \cmdp{q}{\mut a.\cmd{p}{e}}\tau 			  \\[0.3em]

  \cmdf{\injec{i}{V}}{\mut[a_1.c^1\mid a_2.c^2]}\tau	& \reds & c^i_c\tau[a_i:=V] 			 \\
  \cmdf{(V_1,V_2)}{\mut(a_1,a_2).c}\tau 				& \reds & c_c\tau[a_1:=V_1][a_2:=V_2]		 \\
  \cmdf{(V_t,V)}{\mut(x,a).c}\tau 					& \reds & (c[V_t/x])_c\tau[a:=V]			 \\
  \cmdf{\refl}{\muteq.c}\tau 						& \reds & c_c\tau 					 \\[0.5em]\hline

  
  
  \multicolumn{3}{l}{\text{\bf Terms }}\\[-1em]&&\hfill(\text{where $x,a$ are fresh}) \\
  \cmdt{tu}{\pi}\tau          			& \reds & \cmdt{t}{u\cdot \pi}\tau					\\
  \cmdt{S(t)}{\pi}\tau & \reds & \cmdt{t}{\mut x.\cmd{S(x)}{\pi}}	 			\\
  \cmdt{\wit p}{\pi}\tau & \reds & \cmdp{p}{\tmu (x,a).\cut{x}{\pi}}\tau			\\
    \cmdt{\rec{t}{xy}{t_0}{t_S}}{\pi}\tau 	& \reds & \cmdt{t}{\mut z.\cmd{\rec{z}{xy}{t_0}{t_S}}{\pi}}\tau \hfill (t\notin V_t)\\
  \cmdt{\rec{0}{xy}{t_0}{t_S}}{\pi}\tau 	& \reds & \cmdt{t_0}{\pi}\tau 						\\
  \cmdt{\rec{S(V_t)}{xy}{t_0}{t_S}}{\pi}\tau& \reds & \cmdt{t_S[V_t/x][\rec{V_t}{xy}{t_0}{t_S}/y]}{\pi}\tau 	 	\\
  \cmdt{V_t}{\pi}\tau 	      			& \reds & \cmdpi{V_t}{\pi}\tau						\\[0.3em]
  
  
%   \cmdt{\wit p}{\pi}\tau 			& \reds & \cmdp{p}{\mut[a].\cmd{\wit a}{\pi}}\tau 			 \text{ ($a$ fresh)}\\
%   \cmdt{\wit a}{\pi}\tau[a=(t,p)]\tau' 		& \reds & \cmdt{t}{\pi}\tau[a=(t,p)]\tau' 				 \\[0.3em]

  \cmdpi{\lambda x.t}{u\cdot{\pi}}\tau 		& \reds & \cmdt{u}{\mut x.\cmd{t}{\pi}}\tau				 \\
  \cmdpi{V_t}{\mut x .c_t}\tau 			& \reds & (c_t\tau) [V_t/x]						 \\
%   \cmdpi{u}{\mut x.c}\tau 			& \reds & (c_p\tau) [u/x]						 \\
  \cmdpi{V_t}{\mut x .c}\tau 			& \reds & (c_p\tau) [V_t/x]						 \\
  \end{array}$
